A State-Based Characterisation of the Conflict Preorder

This paper proposes a way to effectively compare the potential of processes to cause conflict. In discrete event systems theory, two concurrent systems are said to be in conflict if they can get trapped in a situation where they are both waiting or running endlessly, forever unable to complete their common task. The conflict preorder is a process-algebraic pre-congruence that compares two processes based on their possible conflicts in combination with other processes. This paper improves on previous theoretical descriptions of the conflict preorder by introducing less conflicting pairs as a concrete state-based characterisation. Based on this characterisation, an effective algorithm is presented to determine whether two processes are related according to the conflict preorder.

==> eptcsdata.tex <==
\providecommand{\firstpage}{34}
\providecommand{\publicationstatus}{M.R. Mousavi and A. Ravara: FOCLASA 2011\\
EPTCS 58, 2011, pp.\ \pageref*{FirstPage}--\pageref{LastPage},
doi:\href{http://dx.doi.org/10.4204/EPTCS.58.3}{10.4204/EPTCS.58.3}}

